Active Value Querying to Minimize Additive Error in Subadditive Set Function Learning

Subadditive set functions play a pivotal role in computational economics (especially in combinatorial auctions), combinatorial optimization or artificial intelligence applications such as interpretable machine learning. However, specifying a set function requires assigning values to an exponentially large number of subsets in general, a task that is often resource-intensive in practice, particularly when the values derive from external sources such as retraining of machine learning models. A~simple omission of certain values introduces ambiguity that becomes even more significant when the incomplete set function has to be further optimized over. Motivated by the well-known result about inapproximability of subadditive functions using deterministic value queries with respect to a multiplicative error, we study a problem of approximating an unknown subadditive (or a subclass of thereof) set function with respect to an additive error -- i. e., we aim to efficiently close the distance between minimal and maximal completions. Our contributions are threefold: (i) a thorough exploration of minimal and maximal completions of different classes of set functions with missing values and an analysis of their resulting distance; (ii) the development of methods to minimize this distance over classes of set functions with a known prior, achieved by disclosing values of additional subsets in both offline and online manner; and (iii) empirical demonstrations of the algorithms' performance in practical scenarios.

==> figures/sketch/lower_bound_tikz.tex <==
\begin{tikzpicture}[scale=2]

% Parameters for the logistic curve
\def\a{3} % Maximum value of the logistic curve
\def\b{2}   % Center point (inflection point) of the logistic curve
\def\k{4}   % Steepness of the logistic curve

% Logistic curve (black line) - Concave part only
\draw[thick, domain=2:4, samples=100] plot (\x, {\a/(1 + exp(-\k*(\x-\b)))});

% Red lines (piecewise approximation of the concave part)
\draw[red, thick] (2,{\a/(1 + exp(-\k*(2-\b)))}) -- (2.5,{\a/(1 + exp(-\k*(2.5-\b)))});
\draw[red, thick] (2.5,{\a/(1 + exp(-\k*(2.5-\b)))}) -- (3,{\a/(1 + exp(-\k*(3-\b)))});
\draw[red, thick] (3,{\a/(1 + exp(-\k*(3-\b)))}) -- (3.5,{\a/(1 + exp(-\k*(3.5-\b)))});
% \draw[red, thick] (3.5,{\a/(1 + exp(-\k*(3.5-\b)))}) -- (4,{\a/(1 + exp(-\k*(4-\b)))});

% Blue circles on the concave part of the logistic curve
\foreach \x in {2, 2.5, 3, 3.5} {
    \draw[blue, fill, thick] (\x, {\a/(1 + exp(-\k*(\x-\b)))}) circle [radius=0.03];
}

\end{tikzpicture}

==> figures/sketch/upper_bound_tikz.tex <==
\begin{tikzpicture}[scale=2]

% Parameters for the logistic curve
\def\a{3} % Maximum value of the logistic curve
\def\b{2}   % Center point (inflection point) of the logistic curve
\def\k{4}   % Steepness of the logistic curve

% Logistic curve (black line)
\draw[thick, domain=2:4, samples=100] plot (\x, {\a/(1 + exp(-\k*(\x-\b)))});

\coordinate (I) at (2, {\a/(1 + exp(-\k*(2-\b)))});
\coordinate (J) at (2.15, {\a/(1 + exp(-\k*(2.15-\b)))});
\coordinate (K) at (2.8, {\a/(1 + exp(-\k*(2.8-\b)))});
\coordinate (L) at (3.5, {\a/(1 + exp(-\k*(3.5-\b)))});
\coordinate (M) at (4, {\a/(1 + exp(-\k*(4-\b)))});

% Green lines
\draw[green, thick] (I) -- ($(I)!4!(J)$);
\draw[green, thick] (M) -- ($(M)!2!(K)$);
\draw[green, thick] (M) -- ($(M)!4.2!(L)$);
\draw[green, thick] (L) -- ($(L)!3!(K)$);

% Yellow points
\draw[yellow, fill, thick] ($(I)!2.6!(J)$) circle [radius=0.02];
\draw[yellow, fill, thick] ($(L)!1.4!(K)$) circle [radius=0.02];
\draw[yellow, fill, thick] ($(L)!1.2!(K)$) circle [radius=0.02];

\foreach \x in {I,J, K, L, M} {
    \draw[blue, fill, thick] (\x) circle [radius=0.03];
}

\end{tikzpicture}
